DILEMMA: Joint LLM Quantization and Distributed LLM Inference Over Edge Computing Systems

With a recent trend of using Large Language Models (LLMs) for different applications within smart cities, there is a need for pushing these models toward the edge of network while still preserving their performance. Edge Computing (EC) as a physically closer computing resource to the end users can help to reduce the communication delay for serving end users' tasks for LLM-dependent services. However, EC servers have limited capacity in terms of communication, computation, and storage capacity. This paper introduces DILEMMA, a novel framework addressing the challenges of deploying LLMs in EC systems by jointly optimizing layer placement and layer quantization in EC systems. DILEMMA formulates an Integer Linear Programming problem to minimize total inference delay while ensuring acceptable LLM performance levels, leveraging layer-wise quantization and knowledge distillation for LLM performance control. Experimental evaluations on OPT-350 model using the SQuAD dataset demonstrate that DILEMMA achieves a quantization ratio of up to 12.75% while preserving model loss, highlighting its effectiveness in resource-constrained environments.

==> Sections/Related_work.tex <==
Distributed LLM inference has gained attentions recently due to the large size of the LLMs and their associated computational and memory cost due to autoregressive inference system. Additionally, quantization techniques and their integration into distributed systems can be used for optimizing both system performance and resource utilization. This section reviews the literature on distributed LLM inference, LLM post-training quantization, and joint approaches that combine the two. 

\subsection{Distributed LLM Inference}
Recently, several papers have investigated distributed LLM inference~\cite{wu2023fast, borzunov2024distributed, zhao2024lingualinked, zhang2024edgeshard}. Authors in~\cite{wu2023fast} used parallelization strategies to perform distributed inference serving with multiple GPUs to improve the latency of inference task for LLMs. Borzunov et al.~\cite{borzunov2024distributed} proposed a distributed inference and fine-tuning fault-tolerant method over the Internet. The authors also propose a load balancing algorithm to distribute the load evenly on the devices. LinguaLinked~\cite{zhao2024lingualinked} is proposed by Zhao et al to distribute the LLMs over mobile devices. The authors the LLM to subgraphs and then distribute  subgraphs to mobile devices. The author of work~\cite{wilkins2024online} proposed a distributed LLM inference over data centers to minimize the energy consumption for the inference task. The work~\cite{zhang2024edgeshard} investigated how to jointly partition an LLM and place each partition on multiple edge devices.

\subsection{LLM Quantization}
Quantization~(either pre-training quantization or post-training quantization) can reduce computational cost and memory cost associated with inference task in LLMs. Here, we focus on those papers which used post training quantization~(PTQ).
Several papers have leveraged PTQ to improve the system performance~\cite{xiao2023smoothquant, shao2023omniquant, yuan2023rptq, bai2022towards, li2023fptq}. Xiao et al.~\cite{xiao2023smoothquant} proposed a method to quantize both the activations and the weights to keep the accuracy high while improving the hardware utility. Authors of paper~\cite{shao2023omniquant} proposed a method to optimize the quantization process efficiently for both weight-only and weight-activation quantization by optimizing the clipping threshold. Yuan et al.~\cite{yuan2023rptq} rearrenged the channels and quantize them in clusters to alleviate the impact of range differences between channels. Authors in paper~\cite{bai2022towards} proposed a technique to optimize quantization efficiency by partitioning models into modules, minimizing reconstruction error for each, and applying a parallel training strategy to accelerate quantization. Li et al.~\cite{li2023fptq} employed a layer-wise activation quantization strategy and a novel logarithmic activation equalization method to mitigate quantization errors without requiring fine-tuning.

\subsection{Joint Distributed Inference and LLM Quantization}
Cai et al.~\cite{cai2024edge} proposed a collaborative LLM inference using EC servers while quantizing the LLM. The difference between this work and ours is we partition the LLM into layers and place each layer on an EC server. While this paper~\cite{cai2024edge} uses an EC server as the server and the rest of EC servers as the clients. The server extracts features using the LLM backbone and send the feature
vectors back to the client. This approach is different from ours as we consider a completely distributed system where the cloud server only runs the decision making task.
Zhao et al.~\cite{zhao2024llm} proposed a joint distributed inference and LLM quantization method to reduce the total delay. The authors distribute the LLM layers over a set of GPU servers while quantizing each layer of the LLM. The main difference between our work and paper~\cite{zhao2024llm} is first the objective functions are different. Second, the authors in paper~\cite{zhao2024llm} uses the extra variance of output of a layer due to weight quantization while we use the knowledge distillation to find the difference between the each quantized layer weights and original model weights. Third, the number of decision variables in our DILEMMA problem is less than that of paper~\cite{zhao2024llm}. Therefore, the complexity of our DILEMMA problem is less than that of paper~\cite{zhao2024llm}, making it easily solvable by an off-the-shelf optimization solver. The focus of this work is placing LLM layers on EC servers while quantizing each layer, which does not conflict with GPU-level optimization.

All the previous papers either only considered the distributed LLM inference task~\cite{xiao2023smoothquant, shao2023omniquant, yuan2023rptq, bai2022towards, li2023fptq}, or only considered LLM quantization task~\cite{xiao2023smoothquant, shao2023omniquant, yuan2023rptq, bai2022towards, li2023fptq}, or joint LLM inference and quantization but with a different system setup and LLM performance metric~\cite{cai2024edge, zhao2024llm}. To the best of our knowledge, this is the first work solving joint layer placement and quantization of the LLM over the EC servers with using knowledge distillation concept to control the LLM performance while minimizing total delay in the system.

==> Sections/notation_table.tex <==
\begin{table}[h!]
        \centering
        \caption{Model nomenclature and descriptions.}
        \label{table:notation}
        \begin{tabular}{|c|c|p{0.625\linewidth}|}
            \hline % \toprule \\
            \multicolumn{1}{|c}{} & {\bf Notation} & {\bf Description} \\
            \hline %\midrule
            \parbox[t]{2mm}{\multirow{1}{*}[-12ex]{{\rotatebox[origin=r]{90}{Input Variables}}}}
            & $\mathcal{M}$ & Set of the edge servers indexed by $i$. \\
            \cline{2-3} %\midrule
            & $\mathcal{L}$ & Set of the model layers indexed by $l$. \\
            \cline{2-3}
            & $\mathcal{B}$ & Set of possible bit sizes for quantization indexed by $b$. \\
            \cline{2-3}
            & $p_l$ & The number of output parameters of layer $l \in \mathcal{L}$. \\
            \cline{2-3}
            & $cp_{ilp}$ & The computation capacity required for inference of layer $l$ with $b$ number of parameters at edge server $i$. \\
            \cline{2-3}
            & $cm_{ilp}$ & The communication capacity required for transferring the inference output of layer $l$ with $b$ number of parameters at edge server $i$. \\
            \cline{2-3}
            & $str_{ilp}$ & The storage/memory capacity required for loading layer $l$ with $b$ number of parameters at edge server $i$. \\
            \cline{2-3}
            & $\eta_{i}$ & The communication capacity of edge server $i$.\\
            \cline{2-3}
            & $\gamma_{i}$ & The computation capacity of edge server $i$.\\
            \cline{2-3}
            & $\kappa_{i}$ & The storage/memory capacity of edge server $i$.\\
            \cline{2-3}
            & $P$ & The performance of the LLM model.\\
            \cline{2-3}
            & $P'_{lb}$ & The performance of the qauntized LLM model using $b$ bits parameters at layer $l$.\\
            \hline %
            %% 
            \parbox[t]{2mm}{\multirow{1}{*}[-1.6ex]{{\rotatebox[origin=r]{90}{D.V}}}}
            & $x_{ilb}^t$ & A binary decision variable to show whether the layer $l$ with $b$ parameters will be placed at {edge server} $i$.\\
            \cline{2-3}
            & $y_{ij}$ & A binary decision variable representing the output of layer $l$ placed on edge server $i$ will be sent to edge server $j$ hosting layer $l+1$.\\
            % \cline{2-3}
            % & $t_{ilb}^f$ & A continuous decision variable to show finish time of inference of layer $l$ with $b$ parameters placed at {edge server} $i$.\\
            \hline %
        \end{tabular}
    % \vspace{-6 mm}
    \end{table}
